Design the Feedback, Not Just the Reward: Environments for Open-Ended Reinforcement Learning

Reinforcement learning has advanced large language models on tasks with reliable verifiers, where checking an outcome provides a clear basis for reward. Extending this approach to open-ended tasks requires environments that can both evaluate complex, partially successful outputs and turn these judgments into effective learning guidance. We propose a reinforcement learning framework built around a training environment that integrates human domain knowledge with model reasoning. Human domain knowledge, encoded in rubrics, anchors evaluation to task intent, while model reasoning combined with hierarchical rewards distinguishes complex open-ended outputs and links diagnosed failures to likely responsible output regions. Furthermore, these diagnostic attributions guide token-level weights in the GRPO objective, thereby translating the ambiguous notion of success in open-ended tasks into concrete guidance for policy optimization. We instantiate this framework in interactive web application generation, a representative open-ended generation task. The resulting model achieves an average pass rate of 41.25\% on MiniAppBench and 76.19\% on ArtifactsBench. Ablation studies show the contributions of individual components, while additional out-of-distribution evaluations support transferable gains without degrading performance on other evaluated tasks.

==> _original_backup/section/0_abstract.tex <==
% !TeX root = ../main.tex

\begin{abstract}
\setlength{\parskip}{0.25em}
Interactive web application generation requires models to produce usable HTML, CSS, and JavaScript applications from natural language requests. Unlike conventional code generation, application quality depends on multiple user-facing functional requirements, each often tied to localized code regions such as event handlers, state updates, DOM fragments, or CSS selectors. Standard GRPO collapses these structured outcomes into a single sequence-level reward and applies the resulting advantage uniformly to all tokens, weakening credit assignment. We propose \textbf{Rubric-to-Code Credit Assignment} (RCCA), a reinforcement learning framework that converts rubric-level functional feedback into localized optimization signals over generated code. RCCA builds training tasks around explicit functional rubrics, uses a hierarchical reward to separate format, source-code, runtime, and functional failures, and aligns evaluator-generated textual attributions with responsible code spans and generated tokens. The resulting model, \textbf{Ling-RCCA-Flash}, scores 41.25 on MiniAppBench, improving Ling-3.0-Flash by 32.20 points and slightly surpassing Claude Opus 4.5. It also reaches 76.19 on ArtifactsBench, improving the SFT model by 4.48 points and establishing a new top score under the official ArtifactsBench leaderboard setting by surpassing the GPT-5 score by 3.64 points, suggesting transferable implementation-level gains.
\end{abstract}


==> _original_backup/section/1_introduction.tex <==
% !TeX root = ../main.tex

\section{Introduction}

Large language models are increasingly used to generate software that users can directly see and operate, rather than only text answers or isolated code snippets~\cite{design2code,webcoderbench}. In interactive web application generation, a model takes a natural language request and produces complete HTML, CSS, and JavaScript code for a usable interface~\cite{miniapp,artifactsbench}. This setting introduces a form of correctness that is both user-facing and structured: an application is judged by whether it implements a set of requested behaviors, such as opening a panel after a button click, updating displayed content from an input field, or triggering the correct state transition after an interaction.

This setting also reflects a broader shift from agent infrastructure to model training. Systems such as AWorld~\cite{aworld} provide the harnesses needed to execute agents in realistic environments, observe their behavior, and evaluate task outcomes. In this work, we treat such harnesses not only as evaluation infrastructure, but also as sources of environment-mediated training signals. Interactive web application generation is a natural testbed for this view, because user-visible behaviors can be executed, checked, and often traced back to localized implementation choices. Once an environment exposes interaction traces, requirement-level outcomes, and diagnostic evidence, the central question becomes how to convert these structured signals into effective model updates.

Standard GRPO, however, discards much of this structure~\cite{deepseekr1}. As illustrated in Figure~\ref{fig:intro_motivation}, it collapses multiple functional outcomes into a single sequence-level reward and propagates the resulting group-relative advantage uniformly across all generated tokens, although only a subset of the code may be responsible for a particular success or failure. This creates a mismatch between the granularity of user-facing feedback and the granularity of policy optimization: the model observes whether an application works, but receives little signal about which implementation choices caused it to work or fail.

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{img/intro_figure.png}
  \caption{\textbf{Motivation of RCCA.}
  Standard GRPO collapses rubric-level outcomes into scalar rewards and applies each advantage uniformly to all tokens. RCCA preserves rubric feedback, localizes responsible code spans, and converts them into targeted token weights.}
  \label{fig:intro_motivation}
\end{figure}

We address this mismatch with \emph{Rubric-to-Code Credit Assignment} (RCCA), a reinforcement learning framework that turns user-facing functional rubrics into localized optimization signals over generated code. RCCA is built around task-specific rubrics, where each rubric describes a concrete functional requirement that can be evaluated through interaction. These rubrics serve two roles. First, they guide the construction of RL training tasks with explicit and verifiable behavioral objectives. Second, they provide the evaluation units from which application-level quality can be decomposed into requirement-level outcomes.

To make these outcomes useful for GRPO, RCCA combines sample-level reward discrimination with code-level credit assignment. At the sample level, we design a hierarchical reward that evaluates generated applications through progressively more semantic stages: output-format validity, source-code validity, runtime validity, and rubric-level functional correctness. This hierarchy separates invalid artifacts, broken programs, runtime failures, and partially correct applications, giving group-relative optimization a clearer reward structure than a single holistic score.

At the token level, RCCA further uses textual feedback from the evaluator to identify which code regions are responsible for observed failures or successes. The evaluator not only determines whether each rubric is satisfied, but also attributes the corresponding functional outcome to concrete implementation regions such as event handlers, state updates, DOM fragments, and CSS selectors. RCCA then aligns these attributed code spans with generated tokens and uses them to weight the GRPO objective. As a result, tokens in code regions responsible for functional outcomes receive stronger optimization signals, while unrelated regions are down-weighted. In this way, RCCA restores the missing link between requirement-level feedback and token-level policy updates.

Using the proposed rubric-driven data construction pipeline and RCCA objective, we train \textbf{Ling-RCCA-Flash} for interactive web application generation. As summarized in Figure~\ref{fig:main_results_charts}, it achieves 41.25 on MiniAppBench, improving Ling-3.0-Flash by 32.20 points and slightly surpassing Claude Opus 4.5. It also reaches 76.19 on ArtifactsBench, improving the SFT model by 4.48 points and surpassing the official GPT-5 leaderboard score by 3.64 points. These cross-benchmark gains suggest transferable implementation behavior beyond a single benchmark.

Our contributions are summarized as follows:
\begin{itemize}[leftmargin=*, itemsep=0.15em, topsep=0.25em, parsep=0pt, partopsep=0pt]
\item We construct a high-quality RL dataset for interactive web application generation using a \textbf{rubric-driven synthesis pipeline}, grounding each training task in explicit user-facing functional requirements.

\item We design a \textbf{hierarchical reward} for interactive applications that improves sample-level reward discrimination by separating format, source-code, runtime, and functional failures.

\item We propose \textbf{Rubric-to-Code Credit Assignment} (RCCA), which converts rubric-level functional feedback into localized token-level optimization signals for GRPO through evaluator-generated textual attribution.

\item Using the proposed data and RCCA, we train \textbf{Ling-RCCA-Flash}, which achieves 41.25 on MiniAppBench and 76.19 on ArtifactsBench, demonstrating both target-benchmark gains and cross-benchmark transfer.
\end{itemize}


==> _original_backup/section/2_related_work.tex <==
% !TeX root = ../main.tex
\section{Related Work}

\subsection{Benchmarks for Interactive Web Application Generation}

Traditional code generation benchmarks evaluate functional correctness through programming problems, unit tests, or repository-level edits~\cite{humaneval,mbpp,apps,codecontests,swebench,aider,aider_polyglot}. While effective for measuring isolated coding ability, these benchmarks do not fully capture the quality of user-facing software, where correctness depends not only on code validity but also on visual presentation and interactive behavior.

Recent benchmarks have therefore moved toward web application generation. WebSight and Design2Code focus mainly on static UI generation~\cite{websight,design2code}, while WebDev Arena, ArtifactsBench, MiniAppBench, and DashArena evaluate richer interactive outputs through human preference, visual quality, functional requirements, or dynamic interaction~\cite{webdev_arena,artifactsbench,miniapp,dasharena}. These works highlight that interactive applications should be evaluated as end-to-end user-facing artifacts rather than isolated programs. Our work builds on this shift but focuses on a different question: how to convert structured, requirement-level evaluation into effective training-time reinforcement learning signals. In particular, we use functional rubrics not only to measure application quality, but also to construct RL tasks, decompose application-level outcomes, and support code-localized credit assignment.

\subsection{Fine-Grained Feedback for Language Model Reinforcement Learning}

GRPO improves PPO-style RLHF by estimating a group-relative baseline from multiple sampled responses to the same prompt, avoiding a separate value model~\cite{ppo,instructgpt,deepseekmath,deepseekr1}. However, in interactive web application generation, standard GRPO suffers from a granularity mismatch. Multiple user-facing functional requirements are collapsed into a single sequence-level reward, and the resulting advantage is applied uniformly to all generated tokens. As a result, GRPO may distinguish which sampled application performs better, but it provides little signal about which code regions are responsible for specific functional successes or failures.

Prior work has explored finer supervision through process, segment-level, or token-level feedback~\cite{letsverify,process_reward_models,spo,delta,eapo}, mainly in reasoning and verifiable tasks. Natural language feedback has also been used for critique, revision, policy improvement, and span-level optimization~\cite{rl4f,ilf,reflexion,text2grad}. RCCA differs by treating evaluator-generated textual feedback as a bridge between rubric-level functional outcomes and token-level policy optimization. In interactive HTML/CSS/JavaScript generation, such feedback can often be grounded in concrete implementation regions and local dependencies. RCCA aligns these attributed code regions with generated tokens and uses them to weight the GRPO objective, turning user-facing functional feedback into code-localized credit assignment.

==> _original_backup/section/3_methodology.tex <==
% !TeX root = ../main.tex
\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{img/main_draft.png}
  \caption{\textbf{Overview of RCCA.}
  RCCA assigns credit from rubric-level functional feedback to code regions and optimizes miniapp generation with targeted reinforcement learning signals.}
  \label{fig:method_overview}
\end{figure*}

\section{Method}

\subsection{Problem Formulation and Overview}

We consider interactive web application generation, where a model receives a natural language request $x$ and generates a complete HTML, CSS, and JavaScript application $y$; Figure~\ref{fig:method_overview} provides an overview. Each task is associated with a set of rubrics
\[
\mathcal{R}=\{r_1,\ldots,r_M\},
\]
where each rubric specifies a concrete user-facing requirement, such as an expected initial state or an interaction-triggered behavior. The rubrics serve as the basic units for evaluating requirement satisfaction and attributing outcomes to the generated code.

Standard GRPO assigns each sampled response a sequence-level reward and applies the resulting group-relative advantage uniformly to all generated tokens. This coarse treatment loses useful supervision at both the sample and token levels. At the sample level, applications with different failure modes may receive similar rewards, weakening discrimination within the group. At the token level, the same advantage is applied to the entire response, even when a failure is caused by only a localized code region.

RCCA addresses both limitations. At the sample level, a hierarchical reward distinguishes output-format validity, source-code validity, runtime validity, and rubric-level requirement satisfaction, separating sampled responses more clearly. At the token level, evaluator-generated diagnostics identify code regions associated with detected failures and assign stronger optimization signals to the corresponding tokens. The following sections describe the rubric-driven training data, hierarchical reward, code localization procedure, and RCCA training objective.

\subsection{Rubric-Driven Training Data Construction}

To enable fine-grained evaluation of interactive applications, we construct each training example as a pair $(x,\mathcal{R})$, where $x$ is a natural language request and $\mathcal{R}=\{r_1,\ldots,r_M\}$ is a set of user-facing rubrics describing the expected application state and behavior. Each rubric corresponds to an independently checkable requirement.

We divide the rubrics into two categories according to whether they describe the application's initial state or its behavior under user interaction. \emph{Initial-state} rubrics specify properties that should hold immediately after page load, such as required interface elements, default content, or initial values. \emph{Dynamic} rubrics specify behaviors that should hold after user interaction, such as opening a panel after a click, updating displayed content from an input field, or performing the correct state transition. Initial-state requirements can therefore be verified directly after page load, whereas dynamic requirements require executing the corresponding interaction path.

The same rubric set is used throughout training to evaluate sampled responses, compute the hierarchical reward, and provide requirement-level feedback for code localization. This keeps the supervision used for task construction aligned with the signals used during reinforcement learning and allows failures to be traced from user-facing requirements back to implementation regions.

This design makes each training example both executable and decomposable, allowing failures to be traced from user-facing requirements back to implementation regions.

\subsection{Hierarchical Reward}

Directly aggregating rubric outcomes is insufficient for GRPO because generated applications can fail at qualitatively different stages. A response may violate the output format, contain source-code errors, fail during execution, or remain executable but violate only a subset of user-facing requirements. Treating these cases similarly weakens reward discrimination within the sampled group. We therefore evaluate each response through four stages: (1) \textit{output-format validity}, (2) \textit{source-code validity}, (3) \textit{runtime validity}, and (4) \textit{rubric-level requirement satisfaction}.

Given a response $y$, we first extract the final HTML application and validate its output format. We then inspect the HTML, CSS, and JavaScript for source-level errors that may prevent correct loading, followed by runtime validation of key interaction paths, such as state updates and event chains. Only applications that pass these validity checks proceed to rubric-level evaluation.

We implement this hierarchy as a gated reward:
\[
R(y,\mathcal{R})=
\begin{cases}
0, & F(y)=0,\\
0, & S(y)=0,\\
0.1, & E(y)=0,\\
R_{\mathrm{rubric}}, & \text{otherwise},
\end{cases}
\]
where $F$, $S$, and $E$ indicate whether $y$ passes format, source-code, and runtime validation, respectively, and $R_{\mathrm{rubric}}\in[0.2,1.0]$. The validity gates place fundamentally invalid responses below applications that reach rubric-level evaluation, providing clearer separation for group-relative optimization.

For applications that pass the validity gates, the evaluator checks each rubric independently and identifies violated requirements. Simply counting violations is insufficient: applications that fail the same number of rubrics may differ substantially depending on \emph{which} requirements fail and \emph{how severely}. We therefore associate each rubric with an importance level---\emph{core functionality}, \emph{behavioral correctness}, or \emph{rendering quality}---and assign each violation a severity according to the extent of the failure.

The rubric-level reward is computed as
\[
R_{\mathrm{rubric}}
=
\max\left(
0.2,\,
1-\sum_{r_j\in\mathcal{V}}
p(\ell_j,q_j)
\right),
\]
where $\mathcal{V}$ denotes the set of violated rubrics, $\ell_j$ is the importance level of rubric $r_j$, and $q_j$ is the severity of its violation. The penalty $p(\ell_j,q_j)$ increases with both rubric importance and violation severity.

For severe violations of essential requirements, we additionally impose score ceilings to prevent them from being offset by satisfying less important requirements.


\subsection{Rubric-to-Code Localization}

For each generated application, the evaluator produces a scalar reward together
with diagnostic feedback. The former is computed by the hierarchical procedure
above and determines the response-level advantage in GRPO. The diagnostic feedback consists of a set of issues
\[
\mathcal{D}(y)=\{d_1,\ldots,d_K\},
\]
where each issue arises from \textit{source-code validation}, \textit{runtime validation}, or
\textit{rubric-level requirement checking}. Rubric-level issues are additionally linked
to the corresponding reference rubric. Each issue describes the observed
failure and provides evidence about the relevant implementation, such as code
excerpts, functions, event handlers, state variables, DOM regions, or
interaction paths.

We use this evidence to locate the code associated with each detected error.
Because an interactive behavior may depend on multiple related code regions,
the directly identified evidence may cover only part of the implementation. We
therefore expand the initial locations using source-level relations, including
enclosing functions, event bindings, state reads and writes, and function calls.
This produces a set of localized source spans $\mathcal{S}_k$ for each
diagnostic issue $d_k$.

Finally, we align the localized source spans with the generated token sequence.
For each diagnostic issue $d_k$, we distinguish between code regions directly
related to the detected error and additional regions that are contextually
related through the surrounding implementation. Let
$\mathcal{S}_k^{\mathrm{dir}}$ and $\mathcal{S}_k^{\mathrm{ctx}}$ denote these two
sets of source spans, respectively. These localized regions are converted into
token-level diagnostic weights in the RCCA objective described next.


\subsection{RCCA Training Objective}
To preserve the response-level preference established by the hierarchical reward and avoid distorting it during token-level credit assignment, RCCA applies asymmetric token weighting according to the sign of the advantage. For
negative-advantage responses, the update is concentrated on code regions
associated with detected errors; for positive-advantage responses, these regions
are not further reinforced, while unaffected code receives a slightly stronger
positive update.

Based on the localized regions above, we map character-level spans to completion tokens using the tokenizer offset mapping. Let
$\mathcal{T}^{\mathrm{dir}}$ and $\mathcal{T}^{\mathrm{ctx}}$ denote the tokens whose character spans overlap
$\mathcal{S}^{\mathrm{dir}}$ and $\mathcal{S}^{\mathrm{ctx}}$, respectively. Tokens in
$\mathcal{T}^{\mathrm{dir}}$ receive a diagnostic weight $\bar{w}_{i,t}$ of $3.0$, tokens
in $\mathcal{T}^{\mathrm{ctx}}$ receive $\bar{w}_{i,t}=1.5$, and all other tokens
retain the default weight of $1.0$; the diagnostic weight $\bar{w}_{i,t}$ is
capped at $4.0$. The effective loss weight is then defined as
\[
w_{i,t}
=
\begin{cases}
\bar{w}_{i,t}, & A_i<0,\\
1, & A_i\geq0 \ \text{and}\ 
     t\in\mathcal{T}^{\mathrm{dir}}\cup\mathcal{T}^{\mathrm{ctx}},\\
c, & A_i\geq0 \ \text{and}\ 
     t\notin\mathcal{T}^{\mathrm{dir}}\cup\mathcal{T}^{\mathrm{ctx}},
\end{cases}
\]
where $c=1.2$. This concentrates negative updates on diagnosed error regions while avoiding
additional reinforcement of these regions in positive updates.

We incorporate $w_{i,t}$ into GRPO without altering its group-relative advantage or clipping mechanism. This converts textual diagnostics into token-level gradient weights, directing optimization toward code regions associated with the diagnostic feedback.
\[
\begin{aligned}
&\mathcal{L}_{\mathrm{RCCA}}
= -\frac{1}{G}\sum_{i=1}^{G}\frac{1}{T_i}
  \sum_{t=1}^{T_i}\ell_{i,t},\\
&\ell_{i,t}
= \min\Big(
  \rho_{i,t} w_{i,t} A_i,\,
  \rho^{\mathrm{clip}}_{i,t} w_{i,t} A_i
  \Big),\\
&\rho^{\mathrm{clip}}_{i,t}
= \operatorname{clip}(\rho_{i,t},1-\epsilon,1+\epsilon).
\end{aligned}
\]
where $G$ denotes the number of sampled responses in each GRPO group, $T_i$ is the length of the $i$-th generated response, and $\rho_{i,t}$ is the standard policy probability ratio. Thus, the
hierarchical reward determines the response-level preference, while RCCA
redistributes the resulting optimization signal within each response.


==> _original_backup/section/4_experiment.tex <==
% !TeX root = ../main.tex
\section{Experiment}

\subsection{Experimental Setup}

We apply RCCA to Ling-3.0-Flash, a 124B-parameter hybrid-linear MoE with 5.1B activated parameters per token~\cite{ling3flash}. Starting from this base model, we first perform supervised fine-tuning (SFT) to obtain initial artifact-generation capability, and then conduct RCCA-based reinforcement learning on top of the SFT model. 

We compare these three stages: Ling-3.0-Flash, its SFT variant, and Ling-RCCA-Flash after RCCA, and evaluate them on \textbf{MiniAppBench}~\cite{miniapp}, our primary benchmark for interactive web application generation, and \textbf{ArtifactsBench}~\cite{artifactsbench}, a broader visual and interactive artifact benchmark used to test cross-benchmark generalization.

% This staged comparison isolates gains from SFT-based artifact generation and RCCA-based reinforcement learning.

\subsection{Main Results on MiniAppBench}

\begin{table*}[t]
    \centering
    \caption{\textbf{Main results on MiniAppBench.}
    Pass rates are reported by difficulty and domain, together with average pass rate, token consumption, and inference time when available.}
    \label{tab:miniapp_main}
    \footnotesize
    \setlength{\tabcolsep}{3.5pt}
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\belowcaptionskip}{-4pt}
    \renewcommand{\arraystretch}{1.04}
    \newcommand{\modelicon}[1]{\raisebox{-0.24em}{\includegraphics[height=1.45em]{img/logo_official_png/#1.png}}}
    \newcommand{\anticon}{\raisebox{-0.24em}{\includegraphics[height=1.45em]{img/logo_official_png/ant_ling.png}}}
    \newcommand{\modelgroup}[2]{%
        \multicolumn{14}{@{}c@{}}{%
            \begingroup
            \setlength{\fboxsep}{0.7pt}%
            \colorbox{#1}{\makebox[0.97\textwidth][c]{%
                \raisebox{0pt}[1.35ex][0.25ex]{\textbf{\textit{#2}}}}}%
            \endgroup}\\[1pt]}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{clcccccccccccc}
        \toprule
        \multicolumn{2}{c}{\multirow{3}{*}{Model}} & \multicolumn{9}{c}{Pass Rate (\%)} & \multirow{3}{*}{Avg. (\%)} & \multirow{3}{*}{Tokens} & \multirow{3}{*}{Time(s)} \\
        \cmidrule(lr){3-11}
        \multicolumn{2}{c}{} & \multicolumn{3}{c}{Difficulty} & \multicolumn{6}{c}{Domain} & & & \\
        \cmidrule(lr){3-5}\cmidrule(lr){6-11}
        \multicolumn{2}{c}{} & Easy & Mid & Hard & Games & Science & Tools & Humanities & Viz. & Lifestyle & & & \\
        \midrule
        \modelgroup{yellow!12}{Open-Source Large Language Models}
        \modelicon{qwen} & Qwen3-32B & 1.59 & 0.55 & 0.00 & 0.00 & 0.57 & 0.00 & 0.00 & 2.04 & 3.70 & 0.66 & 3,470.68 & 22.16\\
        \modelicon{qwen} & Qwen3-235B-A22B & 6.43 & 2.35 & 0.00 & 0.93 & 0.60 & 4.00 & 4.88 & 7.27 & 10.34 & 2.88 & 4,068.27 & 49.55\\
        \modelicon{qwen} & Qwen3-Coder-480B-A35B-Instruct & 6.06 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 9.43 & 11.11 & 1.83 & 2,324.83 & 25.04\\
        \modelicon{kimi} & Kimi-K2-Instruct & 14.17 & 5.03 & 0.00 & 3.77 & 3.11 & 4.08 & 4.88 & 17.65 & 18.52 & 6.19 & 3,435.97 & 46.76\\
        \modelicon{zhipu} & GLM-5.1 & 41.50 & 31.40 & 28.50 & 23.70 & 27.70 & 32.10 & 48.60 & 59.60 & 33.30 & 33.50 & -- & --\\
        \midrule
        \modelgroup{blue!10}{Closed-Source Large Language Models}
        \modelicon{hunyuan} & Hunyuan-Turbos-Latest & 6.32 & 0.87 & 0.00 & 0.00 & 0.00 & 3.03 & 0.00 & 13.51 & 3.57 & 2.32 & 3,727.55 & 132.67\\
        \modelicon{xiaomi_mimo} & Mimo-V2-Flash & 28.68 & 8.33 & 2.22 & 13.46 & 6.02 & 10.87 & 11.63 & 23.53 & 36.36 & 12.48 & 5,109.82 & 37.98\\
        \modelicon{grok} & Grok-4.1-Fast-Reasoning & 29.66 & 12.12 & 2.19 & 8.41 & 6.58 & 20.00 & 17.50 & 32.65 & 25.93 & 13.77 & 9,010.00 & 75.62\\
        \modelicon{minimax} & MiniMax-M2.1 & 31.46 & 15.62 & 7.08 & 16.25 & 12.50 & 23.33 & 20.00 & 27.27 & 19.23 & 17.12 & 8,881.57 & 118.32\\
        \modelicon{gemini} & Gemini-3-Flash & 32.76 & 16.89 & 4.10 & 14.95 & 10.60 & 17.95 & 18.18 & 30.61 & 41.38 & 17.62 & 6,563.28 & 50.56\\
        \modelicon{gemini} & Gemini-3-Pro-Preview & 61.98 & 20.83 & 1.71 & 26.74 & 19.11 & 13.64 & 28.57 & 52.00 & 55.56 & 27.52 & 5,815.14 & 80.80\\
        \modelicon{claude} & Claude-Sonnet-4.5 & 68.22 & 14.86 & 1.79 & 16.13 & 22.30 & 29.27 & 23.81 & 47.73 & 44.83 & 26.36 & 8,586.84 & 91.43\\
        \modelicon{claude} & Claude-Opus-4.5 & 59.09 & 41.18 & 22.33 & 37.18 & 34.59 & 47.50 & 35.71 & 57.45 & 56.52 & 41.14 & 13,152.75 & 166.66\\
        \modelicon{openai} & GPT-5.1 & 74.71 & 21.37 & 3.49 & 24.14 & 18.10 & 33.33 & 45.83 & 57.78 & 64.71 & 32.00 & 11,256.15 & 154.09\\
        \midrule
        \modelgroup{green!10}{Ours}
        \anticon & Ling-3.0-Flash & 12.94 & 8.99 & 5.49 & 5.79 & 5.41 & 6.14 & 6.91 & 27.26 & 19.14 & 9.05 & -- & --\\
        \anticon & Ling-3.0-Flash + SFT & 37.41 & 22.45 & 22.44 & 24.17 & 16.04 & 31.58 & 25.53 & 50.00 & 53.12 & 26.85 & -- & --\\
        \anticon & Ling-RCCA-Flash & 53.39 & 35.03 & 37.60 & 39.80 & 29.49 & 24.14 & 54.29 & 63.46 & 70.00 & \textbf{41.25} & -- & --\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-0.6em}
\end{table*}

As shown in Table~\ref{tab:miniapp_main}, Ling-RCCA-Flash achieves an average pass rate of \textbf{41.25\%} on MiniAppBench, slightly above Claude-Opus-4.5 at $41.14\%$ and competitive with the strongest evaluated open-source models. The full training trajectory shows a clear gain: Ling-3.0-Flash obtains $9.05\%$, SFT raises the score to $26.85\%$, and RCCA further improves it by $14.40$ points. Ling-RCCA-Flash also performs strongly across categories, especially on hard tasks ($37.60\%$), Humanities ($54.29\%$), Visualization ($63.46\%$), and Lifestyle ($70.00\%$).

\subsection{Generalization to ArtifactsBench}

We further evaluate Ling-RCCA-Flash on ArtifactsBench, an external benchmark covering a broader range of visual and interactive application-generation tasks.

\begin{table}[t]
    \centering
    \caption{\textbf{ArtifactsBench leaderboard comparison.}
    We insert our evaluated models into the official leaderboard according to
    AVG score; highlighted rows denote our models.}
    \label{tab:artifact_main}
    \small
    \setlength{\tabcolsep}{5pt}
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\belowcaptionskip}{1pt}
    \renewcommand{\arraystretch}{1.09}
    \newcommand{\lbtrophy}{\raisebox{-0.18em}{\includegraphics[height=1.05em]{img/trophy.png}}}
    \newcommand{\lbrank}[2]{\makebox[1.25em][r]{#1}\makebox[1.15em][l]{#2}}
    \newcommand{\lblogo}[1]{\raisebox{-0.20em}{\includegraphics[height=1.1em,width=1.35em,keepaspectratio]{img/logo_official_png/#1.png}}}
    \newcommand{\lbmodel}[2]{\lblogo{#1}\hspace{0.35em}#2}
    \begin{tabular}{@{}>{\centering\arraybackslash}p{0.16\columnwidth}p{0.56\columnwidth}>{\raggedleft\arraybackslash}p{0.16\columnwidth}@{}}
        \toprule
        \rowcolor{black!6}
        \textbf{Rank} & \textbf{Model} & \textbf{AVG $\uparrow$} \\
        \midrule
        \rowcolor{green!15}
        \lbrank{\textbf{1}}{\lbtrophy} & \textbf{\lbmodel{ant_ling}{Ling-RCCA-Flash}} & \textbf{76.19} \\
        \lbrank{2}{} & \lbmodel{openai}{GPT-5} & 72.55 \\
        \rowcolor{green!8}
        \lbrank{3}{} & \lbmodel{ant_ling}{Ling-3.0-Flash + SFT} & 71.71 \\
        \lbrank{4}{} & \lbmodel{minimax}{MiniMax-M2} & 66.80 \\
        \lbrank{5}{} & \lbmodel{claude}{Claude Opus 4.1} & 59.76 \\
        \lbrank{6}{} & \lbmodel{ant_ling}{Ling-1T} & 59.31 \\
        \lbrank{7}{} & \lbmodel{gemini}{Gemini 2.5 Pro} & 57.74 \\
        \lbrank{8}{} & \lbmodel{claude}{Claude Sonnet 4} & 57.28 \\
        \lbrank{9}{} & \lbmodel{openai}{GPT-OSS-120B} & 56.91 \\
        \lbrank{10}{} & \lbmodel{qwen}{Qwen3-235B-A22B-Thinking} & 55.01 \\
        \lbrank{11}{} & \lbmodel{openai}{o3-2025-04-16} & 54.04 \\
        \lbrank{12}{} & \lbmodel{zhipu}{GLM-4.5} & 51.33 \\
        \bottomrule
    \end{tabular}
    \vspace{-0.4em}
\end{table}

As shown in Table~\ref{tab:artifact_main}, Ling-RCCA-Flash reaches \textbf{76.19}, improving the pre-RL model by $4.48$ points and establishing a new top score under the official ArtifactsBench leaderboard setting. It surpasses the top official leaderboard entry, GPT-5 at
$72.55$, by $3.64$ points.

The consistent improvement on this broader benchmark indicates that the benefit of RCCA extends beyond the target MiniAppBench evaluation. By assigning optimization signals to code regions associated with concrete execution and requirement-level feedback, RCCA encourages learning at the level of implementation behavior rather than benchmark-specific output patterns, leading to gains that transfer across related interactive and visual generation tasks.


==> _original_backup/section/5_conclusion.tex <==
% !TeX root = ../main.tex
\section{Conclusion}

We presented Ling-RCCA-Flash, a reinforcement learning approach for interactive web application generation based on Rubric-to-Code Credit Assignment. RCCA addresses the granularity mismatch in standard GRPO by combining hierarchical application-level rewards with token weights derived from rubric-level diagnostic feedback.

Ling-RCCA-Flash achieves 41.25 on MiniAppBench and a state-of-the-art result on ArtifactsBench. These results suggest that applying our hierarchical reward design and assigning credit to responsible implementation regions can improve transferable application-generation behavior across interactive and visual artifact tasks.

More broadly, our results point to a path from agent infrastructure toward model training. By exposing interaction traces, requirement-level outcomes, and localized diagnostics, AWorld-style harnesses produce training signals that RCCA converts into optimization targets for model improvement.


==> _original_backup/section/6_limitations.tex <==
% !TeX root = ../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1. Limitations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Limitations}

Ling-RCCA-Flash focuses on interactive HTML/CSS/JavaScript application generation and is evaluated on MiniAppBench and ArtifactsBench. The current evaluation does not fully cover large multi-page applications, backend services, persistent storage, authentication flows, or production deployment constraints. RCCA also relies on evaluator-generated rubric judgments and textual attributions; incorrect diagnostics may assign credit to the wrong implementation spans, especially when failures arise from interactions among distant code regions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2. Ethics Statement
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Ethics Statement}

In this work, we propose Ling-RCCA-Flash for generating interactive web applications from natural language requests. We adhere to the ACL Code of Ethics and highlight the following:

\begin{itemize}
    \item \textbf{Data Privacy:} The training and evaluation data are constructed from benchmark tasks and synthesized rubrics rather than private user data, and we avoid intentionally including personally identifiable information.
    
    \item \textbf{Responsible Application Generation:} Generated applications may contain functional, security, or accessibility defects. Ling-RCCA-Flash is intended for prototyping and research evaluation, and generated code should be inspected before deployment.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 3. Acknowledgements
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Acknowledgements}

The authors thank colleagues at Inclusion AI and Ant Group for helpful discussions and infrastructure support. We acknowledge the use of generative AI tools for polishing the linguistic quality and refining the prose of this manuscript. All technical claims and final content remain the sole responsibility of the authors.


==> section/6b_ai_disclosure.tex <==
\section*{AI Use Disclosure}

In this work, we used generative AI tools in two ways: as part of the proposed research framework and as writing assistance during manuscript preparation.

First, LLMs are part of the training environment studied in this paper. They are used to support rubric construction, including controlled query expansion, requirement extraction, functional module grouping, atomic rubric decomposition, and final rubric filtering under human-specified construction rules. LLMs are also used as code-based diagnostic judges during reward computation, where they identify static issues, code-inferred executability issues, and rubric-alignment deficiencies from generated HTML/CSS/JavaScript source code. These uses are described as part of the method, and the resulting feedback is converted into scalar rewards and diagnostic token weights by deterministic post-processing code.

Second, generative AI tools were used to assist the authors in preparing the manuscript. This assistance included drafting and revising paragraphs, improving English readability, translating author-written Chinese notes into English, reorganizing appendix material, checking consistency between the main text and appendix, and formatting LaTeX equations and tables. The authors reviewed, edited, and verified all AI-assisted text.

We did not use generative AI tools to fabricate experimental results, create unsupported claims, or replace author verification of the methodology, formulas, experiments, or conclusions. All reported experimental results, model configurations, reward definitions, and benchmark numbers were checked by the authors. The authors take full responsibility for the final content of the paper, including any text, claims, data, or artifacts produced with the assistance of generative AI.

